Quantum Fisher Information and its dynamical nature

The importance of the quantum Fisher information metric is testified by the number of applications that this has in very different fields, ranging from hypothesis testing to metrology, passing through thermodynamics. Still, from the rich range of possible quantum Fisher information, only a handful are typically used and studied. This review aims at collecting a number of results scattered in the literature that can be useful to people who begin the study of Fisher information and to those who are already working on it to have a more organic understanding of the topic. Moreover, we complement the review with new results about the relation between Fisher information and physical evolutions. Extending the study done in [1], we prove that all the physically realisable dynamics can be defined solely in terms of their relation with respect to the Fisher information metric. Moreover, other properties as Markovianity, retrodiction or detailed balance can be expressed in the same formalism. These results show a fact that was partially overseen in the literature, namely the inherently dynamical nature of Fisher information.

==> appendices.tex <==
\section{Properties of the contrast functions}
We can now explore which constraints have to be imposed on $g(x)$ to satisfy the requirements above. The positivity condition~\ref{cf:item:positivity} corresponds to imposing that $g(1)=0$ is the only zero of the function. Moreover, by noticing the fact that the contrast function associated to $g(x) = (x-1)$ is identically zero (as $H_g(\rho||\sigma) = \Tr{\sigma - \rho}\equiv 0$) in order to ensure the positivity of $H_g(\rho||\sigma)$ it is sufficient to require that $g(x) + a(x-1)\geq 0$, for some arbitrary  constant $a$. On the other hand, condition~\ref{cf:item:homogeneity} is automatically satisfied, while one needs to require that $g(x)$ is matrix convex at $x = 1$ for the joint convexity to hold (condition~\ref{cf:item:jointConvexity}). This directly implies  the monotonicity of the contrast functions, condition~\ref{cf:item:monotonicity}, fact that can be proved as follows: first, it should be noticed that $H_g(\rho||\sigma)$ are unitary invariant. Indeed, one has:
\begin{align}
	H_g (U\,\rho\,U^\dagger||U\,\sigma\,U^\dagger) :&= \Tr{U\,\rho^{1/2}\,U^\dagger\, g\boldsymbol{(}\LL_{U\,\sigma\,U^\dagger}\RR_{U\,\rho^{-1}\,U^\dagger}\boldsymbol{)}\sqrbra{U\,\rho^{1/2}\,U^\dagger}} =\label{cf:eq:127n}\\
	&=\Tr{U\,\rho^{1/2}\,U^\dagger\,U\, g\boldsymbol{(}\LL_{\sigma}\RR^{-1}_{\rho^{-1}}\boldsymbol{)}\sqrbra{\rho^{1/2}}\,U^\dagger} = H_g (\rho||\sigma) \,,\label{cf:eq:128n}
\end{align}
where the step from Eq.~\eqref{cf:eq:127n} to the Eq.~\eqref{cf:eq:128n} can be verified either in coordinates (see Eq.~\eqref{cf:eq:HGCoordinateExpression}), or by expanding $g(x)$ in Laurent series, while in Eq.~\eqref{cf:eq:128n} we exploited the unitarity of $U$ and the cyclicity of the trace. Second, also notice that for generic contrast functions it holds that:
\begin{align}
	H_g (\rho\otimes\tau||\sigma\otimes\tau) &= \Tr{ g\boldsymbol{(}\LL_{\sigma\otimes\tau}\RR_{\rho\otimes\tau}^{-1}\boldsymbol{)}\sqrbra{\rho\otimes\tau}} = \Tr{ (g\boldsymbol{(}\LL_{\sigma}\RR_{\rho}^{-1}\boldsymbol{)}\otimes\idO)\sqrbra{\rho\otimes\tau}}=\label{cf:eq:130B}\\
	&= \Tr{ g\boldsymbol{(}\LL_{\sigma}\RR_{\rho}^{-1}\boldsymbol{)}\sqrbra{\rho}}\Tr{\tau}= H_g (\rho||\sigma)\label{cf:eq:131n}\,,
\end{align}
where in Eq.~\eqref{cf:eq:130B} we used the fact that $\LL_\tau\RR_\tau^{-1}$ coincides with the identity operator on the commutant of $\tau$, together with the fact that $g(1) = 1$. This identity can also be verified by expanding $g(x)$ in Laurent series. These two facts allow to deduce the monotonicity of the contrast functions in Eq.~\eqref{cf:eq:HGexpressionApp} from their joint convexity. Indeed, given a CPTP map $\Phi$, one can express it in terms of its Stinespring's dilation:
\begin{align}\label{cf:eq:stinespring}
	\Phi(\rho) = \TrR{E}{U\, (\rho \otimes \ketbra{\psi}{\psi})\,U^\dagger}\,,
\end{align}
where $U$ is a unitary operator and $\ketbra{\psi}{\psi}$ is an environmental pure state of dimension $d_E$. Take a unitary basis $\{V_i\}$ for the space of bounded operators of dimension $d_E^2$. It is a well-known result that $\sum_i (V_i(\rho_E)V_i^\dagger)/d_E^2 = \id_E/d_E$ for any $\rho_E$~\cite{nielsen2002quantum}. We denote this operator by $\Delta_1(\rho)$. This identity, together with Eq.~\eqref{cf:eq:stinespring} allows us to rewrite the action of the channel as:
\begin{align}\label{cf:eq:130n}
	\Phi(\rho)\otimes \frac{\id_{d_E}}{d_E} = \frac{1}{d_E^2} \,\sum_{i=1}^{d_E^2} \; (\idO\otimes V_i)U\, (\rho \otimes \ketbra{\psi}{\psi})\,U^\dagger(\idO\otimes V_i^\dagger)\,,
\end{align}
where we used $\id$ to indicate the identity matrix, and $\idO$ for the identity superoperator.
Putting together this expression with Eq.~\eqref{cf:eq:131n} we can finally prove monotonicity. Indeed, one has:
\begin{align}
	&H_g(\Phi(\rho)||\Phi(\sigma)) = H_g\norbra{\Phi(\rho)\otimes \frac{\id_{d_E}}{d_E} \bigg|\bigg|\Phi(\sigma)\otimes \frac{\id_{d_E}}{d_E} } = \\
	&\!= H_g\norbra{(\id\otimes\Delta_1)\norbra{U\, (\rho \otimes \ketbra{\psi}{\psi})\,U^\dagger}||(\id\otimes\Delta_1)\norbra{U\, (\sigma \otimes \ketbra{\psi}{\psi})\,U^\dagger}} \leq\\
	&\leq \frac{1}{d_E^2} \,\sum_{i=1}^{d_E^2} \;H_g(\rho \otimes \ketbra{\psi}{\psi}||\sigma \otimes \ketbra{\psi}{\psi}) =H_g(\rho ||\sigma ) \,,\label{cf:eq:36}
\end{align}
where in the first line and in the third line we used Eq.~\eqref{cf:eq:131n}, while in the step from the second to the third line we used the decomposition in Eq.~\eqref{cf:eq:130n} together with the unitary invariance and joint convexity of $H_g$. This proves condition~\ref{cf:item:monotonicity}.

\section{Derivation of the flux of Fisher information}\label{app:sec:fisherFlow}

We present here the derivation of Thm.~\ref{cf:thm:FisherFlow}. In particular, we want to study the evolution of the Fisher information:
\begin{align}
	\mathcal{F}_t:= \Tr{\delta\rho_t\,\J_f^{-1}\big|_{\pi_t} [\delta\rho_t]}\,,
\end{align}
where $\pi_t := \Phi_t(\pi)$ and $\delta\rho_t := \Phi_t(\delta\rho)$. Using the integral expression in Eq.~\eqref{cf:eq:thm2HGexpIntegral}, we can rewrite the Fisher information as:
\begin{align}
	\mathcal{F}_t = 2\,{\rm Re}\int_0^1 \de N_g (s)\; \Tr{\delta\rho_t\, (\LL_{\pi_t}+s\,\RR_{\pi_t})^{-1}[\delta\rho_t]}\,,
\end{align}
where the real part comes from the fact that $(\LL_\pi + s \RR_\pi)^{\dagger}=(\RR_\pi + s \LL_\pi)$. This expression is particularly convenient for calculations, due to the simple form that the derivative of $(\LL_{\pi_t}+s\,\RR_{\pi_t})^{-1}$ takes. In fact, this is given by:
\begin{align}\label{appM:eq:3}
	\frac{\de}{\dt}(\LL_{\pi_t}+s\,\RR_{\pi_t})^{-1} = - (\LL_{\pi_t}+s\,\RR_{\pi_t})^{-1}(\LL_{\dot\pi_t}+s\,\RR_{\dot\pi_t})(\LL_{\pi_t}+s\,\RR_{\pi_t})^{-1}\,,
\end{align}
where $\dot \pi_t$ is simply the derivative of the state. This expression can be proved by noticing that $\frac{\de}{\dt}\LL_{\pi_t} = \LL_{\dot{\pi}_t}$ (and similarly for $\RR_{\pi_t}$) and by taking the derivative of:
\begin{align}
	\frac{\de}{\dt}\norbra{(\LL_{\pi_t}+s\,\RR_{\pi_t})(\LL_{\pi_t}+s\,\RR_{\pi_t})^{-1}} &= (\LL_{\dot{\pi}_t}+s\,\RR_{\dot{\pi}_t})(\LL_{\pi_t}+s\,\RR_{\pi_t})^{-1} +(\LL_{\pi_t}+s\,\RR_{\pi_t})\frac{\de}{\dt}(\LL_{\pi_t}+s\,\RR_{\pi_t})^{-1}=\\
	&= \frac{\de}{\dt} \,\idO = 0\,,
\end{align}
which directly implies Eq.~\eqref{appM:eq:3}. Given this technical tool, we can start analysing the evolution of $\mathcal{F}_t$ under the dynamics generated by the Lindbladian:
\begin{align}
	\lind_t[\rho] = -i[H_t,\rho] + \sum_{\alpha}^{d^2} \;\lambda_\alpha\,\norbra{A_\alpha(t) \,\rho\, A_\alpha(t)^\dagger - \frac{1}{2}\{A_\alpha(t)^\dagger \,A_\alpha(t), \rho\}}\,.
\end{align}
Notice that, since $\mathcal{F}_t$ is invariant under unitary transformations, there is no contribution coming from the commutator in the previous equation. Moreover, since the derivative is linear, it decomposes into a sum of the form:
\begin{align}
	\dot{\mathcal{F}_t} = \sum_\alpha\; \lambda_\alpha(t)\, \,\mathcal{I}_\alpha(t)\,,
\end{align}
where each current $\mathcal{I}_\alpha(t)$ only contains the corresponding jump operator $A_\alpha(t)$, together with its adjoint. For this reason, without loss of generality, we consider here Lindblad operators generated by a single jump operator. In order to shorten the notation we also assume that the jump operator, denoted by $A$, is time independent, again without loss of generality. We start by rewriting the derivative of the Fisher information as:
\begin{align}
	\dot{\mathcal{F}_t}=2\,{\rm Re}\int_0^1 \de N_g (s)\; \bigg (2\, &\Tr{\delta\dot\rho_t (\LL_{\pi_t}+s\,\RR_{\pi_t})^{-1}[\delta\rho_t]} + \Tr{\delta\rho_t \norbra{\frac{\de}{\dt}(\LL_{\pi_t}+s\,\RR_{\pi_t})^{-1} }[\delta\rho_t]}\bigg )\,.\label{appM:eq:9}
\end{align}
The second term in the integral  can be expanded as:
\begin{align}
	\Tr{\delta\rho_t \norbra{ \frac{\de}{\dt}(\LL_{\pi_t}+s\,\RR_{\pi_t})^{-1} }[\delta\rho_t]} &=- \Tr{\delta\rho_t (\LL_{\pi_t}+s\,\RR_{\pi_t})^{-1}(\LL_{\dot\pi_t}+s\,\RR_{\dot\pi_t})(\LL_{\pi_t}+s\,\RR_{\pi_t})^{-1}[\delta\rho_t]} = \\
	&= - \Tr{B_{s}(t)^\dagger \,\dot\pi_t \,B_{s}(t)} - s\, \Tr{B_{s}(t)^\dagger  B_{s}(t)\,\dot\pi_t} =\\
	&= - \Tr{B_{s}(t)^\dagger \,\lind({\pi_t}) \,B_{s}(t)} - s\, \Tr{B_{s}(t)^\dagger  B_{s}(t)\,\lind({\pi_t}) }\,,\label{cf:eq:B8}
\end{align}
where we introduced the notation $B_{s}(t) := (\LL_{\pi_t}+s\,\RR_{\pi_t})^{-1}[\delta\rho_t]$.  On the other hand, the first term in Eq.~\eqref{appM:eq:9} simply gives:
\begin{align}
	2\, \Tr{\delta\dot\rho_t (\LL_{\pi_t}+s\,\RR_{\pi_t})^{-1}[\delta\rho_t]} =
	&= 2 \,\Tr{\lind(\delta\rho_t) B_{s}(t)} = 2\, \Tr{\lind((\RR_{\pi_t}+s\,\LL_{\pi_t})[ B_{s}(t)^\dagger])  B_{s}(t)}=\\
	&=2 \,\Tr{\lind( B_{s}(t)^\dagger \pi_t) B_{s}(t)} + 2s\, \Tr{\lind(\pi_t  B_{s}(t)^\dagger ) B_{s}(t)}\,,\label{cf:eq:B10}
\end{align}
where in the first line we have multiplied and divided by $(\RR_{\pi_t}+s\,\LL_{\pi_t})$ to obtain $ B_{s}(t)^\dagger $. We can now proceed in summing up Eq.~\eqref{cf:eq:B8} and Eq.~\eqref{cf:eq:B10}. Due to the number of terms that will appear, though, we first consider the first traces in both equations, and then the second ones. Hence, summing the first term in  Eq.~\eqref{cf:eq:B8} and the first of Eq.~\eqref{cf:eq:B10}, and explicitly expanding the Lindbladian, we obtain:
\begin{align}
	&2 \,\Tr{A\, B_{s}(t)^\dagger \pi_tA^\dagger  B_{s}(t)} - \cancel{\Tr{ B_{s}(t)^\dagger \pi_tA^\dagger A\,  B_{s}(t)}}-  \Tr{A^\dagger A\, B_{s}(t)^\dagger \pi_t B_{s}(t)} +\nonumber\\
	&- \Tr{ B_{s}(t)^\dagger A\,\pi_t A^\dagger\,  B_{s}(t)} +\cancel{\frac{1}{2} \Tr{ B_{s}(t)^\dagger\pi_t A^\dagger A\,  B_{s}(t)}}+\cancel{\frac{1}{2} \Tr{ B_{s}(t)^\dagger A^\dagger A\,\pi_t   B_{s}(t)}}\,,
\end{align}
where the first three terms come from Eq.~\eqref{cf:eq:B8}, and the last three from Eq.~\eqref{cf:eq:B10}.
Notice that the second term corresponding to Eq.~\eqref{cf:eq:B8} cancels with the last two terms coming from Eq.~\eqref{cf:eq:B10}. Indeed, we can take the conjugate of the last trace without affecting the result, thanks to the real part in Eq.~\eqref{appM:eq:9}.  The remaining terms can be further simplified to give:
\begin{align}
	2&\Tr{\pi_tA^\dagger  B_{s}(t)A\, B_{s}(t)^\dagger } -  \Tr{ \pi_t B_{s}(t)A^\dagger A\, B_{s}(t)^\dagger}- \Tr{\pi_t A^\dagger\,  B_{s}(t) B_{s}(t)^\dagger A} =\\
	&\qquad= \Tr{\pi_t\,[A^\dagger,  B_{s}(t)]\,A B_{s}(t)^\dagger } + \Tr{\pi_t\,A^\dagger  B_{s}(t)\,[A, B_{s}(t)^\dagger] }=\\
	&\qquad= -\Tr{\pi_t\, B_{s}(t)A^\dagger\,[A,  B_{s}(t)^\dagger]} + \Tr{\pi_t\,A^\dagger  B_{s}(t)\,[A, B_{s}(t)^\dagger] } =\\
	&\qquad=\Tr{\pi_t\,[A^\dagger,  B_{s}(t)][A, B_{s}(t)^\dagger] } =\\
	&\qquad= -  \Tr{\pi_t\,[A,  B_{s}(t)^\dagger]^\dagger[A, B_{s}(t)^\dagger] }\,, 
\end{align}
where in the first line we used the cyclicity of the trace to put in evidence $\pi_t$, then in the third line we took the complex conjugate of the trace (again exploiting the fact that only the real part contributes to the Fisher information), and used the identity $[X,Y]^\dagger = [Y^\dagger,X^\dagger] =-[X^\dagger,Y^\dagger] $.

We can now pass to examine the last two terms in Eq.~\eqref{cf:eq:B8} and Eq.~\eqref{cf:eq:B10}. Since the steps are completely analogous to the ones in the previous derivation, we present them all together. Carrying them out gives:
\begin{align}
	&2s\, \Tr{A\pi_t  B_{s}(t)^\dagger A^\dagger  B_{s}(t)} - \cancel{s\Tr{A^\dagger A\pi_t  B_{s}(t)^\dagger  B_{s}(t)}}
	- s\,\Tr{\pi_t  B_{s}(t)^\dagger A^\dagger A\, B_{s}(t)} +\\
	&- s\, \Tr{ B_{s}(t)^\dagger   B_{s}(t)A\pi_tA^\dagger}+\cancel{\frac {s}{2}\, \Tr{ B_{s}(t)^\dagger   B_{s}(t)A^\dagger A\pi_t}}+\cancel{\frac {s}{2}\, \Tr{ B_{s}(t)^\dagger   B_{s}(t)\pi_tA^\dagger A}} = \\
	%&= 2s\, \Tr{\pi_t  B_{s}(t)^\dagger A^\dagger  B_{s}(t)A} - s\,\Tr{\pi_t  B_{s}(t)^\dagger A^\dagger A\, B_{s}(t)}- s\, \Tr{\pi_tA^\dagger  B_{s}(t)^\dagger   B_{s}(t)A} = \\
	&= s\, \Tr{\pi_t \,[ B_{s}(t)^\dagger, A^\dagger ] \,B_{s}(t)A}+s\, \Tr{\pi_t\,  B_{s}(t)^\dagger A^\dagger\, [ B_{s}(t),A]} =\\
	&= - s\, \Tr{\pi_t \,A^\dagger  B_{s}(t)^\dagger\, [ B_{s}(t), A ]} +s\, \Tr{\pi_t \, B_{s}(t)^\dagger A^\dagger\, [ B_{s}(t),A]}=\\ 
	&= s\, \Tr{\pi_t\, [ B_{s}(t)^\dagger, A^\dagger] [ B_{s}(t),A]} =\\
	&= -s\, \Tr{\pi_t\, [ B_{s}(t), A]^\dagger [ B_{s}(t),A]}=\\
	& = -s\, \Tr{\pi_t \,[A, B_{s}(t)]^\dagger [A, B_{s}(t)]} \,.
\end{align}
This concludes the proof of Thm.~\ref{cf:thm:FisherFlow}. In fact, generalising again to the case of many time dependent jump operators, we finally obtain:
\begin{align}
	&\dot{\mathcal{F}_t} = \sum_\alpha\; \lambda_\alpha(t)\, \,\mathcal{I}_\alpha(t)= \\
	&=-2\, \sum_\alpha\; \lambda_\alpha(t)\,\int_0^1 \de N_g (s)\; \bigg(\Tr{\pi_t\,[A_\alpha(t),  B_{s}(t)^\dagger]^\dagger[A_\alpha(t), B_{s}(t)^\dagger] } +s\, \Tr{\pi_t\, [A_\alpha(t), B_{s}(t)]^\dagger [A_\alpha(t), B_{s}(t)]} \bigg)\,,
\end{align}
where we can drop the real part, as both the terms in the integral are positive definite.

\section{Markovianity for classical evolutions}\label{app:markovianEvolutions}

Classical dissipative evolutions are described by stochastic maps, i.e., matrices $\Phi$ satisfying the two conditions:
\begin{align}
	&\sum_{i}\;(\Phi)_{i,j} = 1\label{appM:eq:T_require}\,;\\
	&(\Phi)_{i,j} \geq 0\qquad \forall\;\; \{i,j\}\,,\label{appM:eq:T_requireP}
\end{align}
where the first condition ensures the conservation of total probability, while the second is needed to make sure that states are mapped into states.
In complete analogy to the quantum case, a family of stochastic maps $\Phi_t$ depending smoothly on $t$ is called divisible if for any two times $t$ and $s$ ($t\geq s$) one can define an intermediate map $\Phi_{t,s}$ satisfying the relation $\Phi_{t} = \Phi_{t,s}\circ\Phi_s$. A divisible stochastic dynamics is Markovian if all the intermediate maps $\Phi_{t,s}$ are stochastic.

The smoothness in $t$ allows to define the rate matrix $R_t$ through the equation
\begin{align}
	R_t:=\lim_{\varepsilon\rightarrow 0}\,\frac{\Phi_{t+\varepsilon,t} - \idO}{\varepsilon}\,.
\end{align}
Then, since the composition of two stochastic maps is again stochastic, Markovianity holds if and only if $R_t$ generates a stochastic evolution for any time $t$. For this reason, it is useful to characterise this kind of rate matrices. To this end, consider the matrix $\Phi_{t+\varepsilon,t}\simeq \idO + \varepsilon\,R_t$. For the global evolution to be Markovian, this matrix should satisfy the two conditions in Eq.~\eqref{appM:eq:T_require} and Eq.~\eqref{appM:eq:T_requireP}, namely:
\begin{align}
	&\sum_i \;\norbra{\delta_{ij} +\varepsilon\, (R_t)_{i,j}} = 1+\varepsilon\, \sum_i \; (R_t)_{i,j} = 1\,,\label{cf:eq:Rate_conditions}\\
	&\delta_{ij} + \varepsilon\, (R_t)_{i,j}\geq 0 \qquad\forall\;\; \{i,j\}\,,\label{cf:eq:Rate_conditions2}
\end{align}
where $\delta_{ij}$ denotes the Kronecker delta. From the first condition we can deduce that $\sum_i  (R_t)_{i,j} = 0$. In particular, highlighting the diagonal terms, one obtains $R_{j,j}^{(t)} = -\sum_{i\neq j}  R_{i,j}^{(t)} $. Matrices satisfying this constraint can be decomposed as:
\begin{align}
	R_t=\sum_{i\neq j} \; a^{(t)}_{i\leftarrow j}\left( \ketbra{i}{j}-\ketbra{j}{j} \right)\label{appM:rateMatrixTracePreserving}
\end{align}
for $a^{(t)}_{i\leftarrow j}$ some real coefficients. We assume that this condition is always satisfied, also for non-Markovian evolutions, as it corresponds to the requirement that the dynamics preserves the normalisation. In fact, since non-Markovian evolutions are trace preserving on their domain, one can argue by linearity that this condition can be extended to the whole space of states.

Moreover, the condition in Eq.~\eqref{cf:eq:Rate_conditions2} implies that $ (R_t)_{i,j}\geq 0$ whenever $i\neq j$. In the parametrisation above this means that the rates satisfy $a^{(t)}_{i\leftarrow j}\geq 0$. Hence, Markovianity corresponds to the request of having positive rates $a^{(t)}_{i\leftarrow j}$ for all times. 

It should be pointed out that the derivation just presented is completely analogous  to the one for the Lindbladian operators. In fact, in the same way we characterised trace preserving maps with Thm.~\ref{cf:thm:tracePreservingMaps}, one needs to do the same for stochastic matrices, leading to Eq.~\eqref{appM:rateMatrixTracePreserving}. Once this parametrisation is obtained, it is then straightforward to connect Markovianity and positivity of rates.

\section{Use of the trace distance in non-Markovianity}\label{app:sec:fisherAndTrace}

The study of non-Markovianity is mainly carried out in terms of information quantifiers, like, for example, distinguishability distances. These are functions devised to quantify how statistically distinguishable two states are, and they usually
decrease under physical evolutions. Then, as this leads to a monotonic decrease in these distances under Markovian dynamics, any increase thereof signals the appearance of non-Markovianity. In this context, the most used example is given by the trace distance:
\begin{align}
	D_{\rm Tr}(\rho,\sigma)=\Tr{|\rho-\sigma|}\,.
\end{align}
This quantity is connected to the maximal probability $p_d$ of distinguishing $\rho$ from $\sigma$ in a single shot measurement, thanks to the relation $p_d (\rho,\sigma)= (1+D_{\rm Tr}(\rho,\sigma))/2$~\cite{nielsen2002quantum}. Moreover, since it is translational invariant, it is particularly appealing for analytical calculations. In particular, suppose $\rho$ and $\sigma$ are two probability vectors, and define $\delta\rho := \sigma-\rho$. Then, the trace distance is given by:
\begin{align}
	D_{\rm Tr}(\rho,\sigma) =D_{\rm Tr}(\rho,\rho + \delta\rho) = \Tr{|\delta\rho|}\,.
\end{align}
If the evolution is described by the rate matrix $R_t$, it is straightforward to see that:
\begin{align}
	\frac{\de}{\dt}\, D_{\rm Tr}(\rho,\sigma) &= \frac{\de}{\dt}\,\Tr{|\delta\rho|}=\sum_i   \;\frac{\de}{\dt} |{\delta\rho_i}| = \sum_i  \;{\rm sign}(\delta\rho_i) \delta\dot{\rho_i}=\\
	&=\sum_i  {\rm sign}(\delta\rho_i)  \sum_{j} \,(R_t)_{i,j}\, d_j =\sum_{i\neq j} \;{\rm sign}(\delta\rho_i)\left(a_{i\leftarrow j}^{(t)}\delta\rho_j - a_{j\leftarrow i}^{(t)}\delta\rho_i\right)=\\
	&=\sum_{i\neq j} \;a_{j\leftarrow i}^{(t)}\,\delta\rho_i \left({\rm sign}(\delta\rho_j)- {\rm sign}(\delta\rho_i)\right)\,.
\end{align}
where we used the parametrisation of the rate matrix in Eq.~\eqref{appM:rateMatrixTracePreserving}, and in the last line we swapped the indexes of the first term in order to put the coefficient $a_{j\leftarrow i}^{(t)}$ in evidence. It should be noticed that if all the rates are positive, then the sum will be negative: in fact, either ${\rm sign}(\delta\rho_j)= {\rm sign}(\delta\rho_i)$, in which case the term inside the parenthesis is zero, or ${\rm sign}(\delta\rho_j)= -{\rm sign}(\delta\rho_i)$, so that $\delta\rho_i({\rm sign}(\delta\rho_j)- {\rm sign}(\delta\rho_i))=-2\,\delta\rho_i\,{\rm sign}(\delta\rho_i)=-2|\delta\rho_i|$. 
This calculation shows explicitly how the trace distance decreases under Markovian maps. 

Interestingly, it is a well known fact that an evolution is Markovian if and only if the trace norm of any vector $\boldsymbol{v}$ decreases monotonically~\cite{rivas2014quantum}. For this reason, it would be natural to expect the same to hold for the trace distance as well. It is easy to see, though, that this is false: one simple counterexample can be given in dimension $d=2$, with $a_{1\leftarrow 2}<0$ and $a_{2\leftarrow 1}>0$, and the additional condition that $|a_{2\leftarrow 1}|>|a_{1\leftarrow 2}|$. Plugging such choice in Eq.~\eqref{eqapp:trace_deriv}, and using the fact that in dimension $2$ in order for  $\delta\rho$ to be traceless it must satisfy $\delta\rho_1=-\delta\rho_2$, it is easy to check that the derivative of the trace distance stays negative. Still, there is no contradiction between the two results: indeed, the trace distance can only access vectors of the form $\delta \rho= \sigma-\rho$, i.e., that are traceless. This reduces the dimension of the vectors tested by one. In fact, by choosing the traceful vector $v_i=\delta_{i2}$, one is able to witness non-Markovianity in the counterexample just presented.

Suppose now to have access to extra ancillary degrees of freedom on which the dynamics acts trivially, i.e., the global evolution is given by $\Phi_t\otimes\idO_{d_A}$, where $d_A$ is the dimension of the ancilla. Then, one can always find product states $\rho$ and $\sigma$ on the composite space such that $\TrR{S}{\rho-\sigma} \neq 0$ while $\TrR{A}{\rho-\sigma} = 0$, so that the total trace is zero. In this way, ancillary degrees of freedom give access to traceful vectors, and so to the possibility of witnessing non-Markovianity. A similar argument was also presented in~\cite{bylicka2017constructive} for the case of quantum dynamics. These results lead to the following:
\begin{theorem}
	\label{lem:ancilla}
	Given a divisible dynamics $\Phi_t$, there always exists an ancilla of finite dimension $d_A$ on which the dynamics acts trivially (i.e., the total evolution is given by $\Phi_t\otimes\idO_{d_A}$) such that one can witness any non-Markovianity in $\Phi_t$ via revivals in the trace distance between initially prepared states.
\end{theorem}

For quantum states $d_A = d+1$~\cite{bylicka2017constructive}. It should be noticed, though, that in order to actually speak about complete positivity one always needs an ancilla of dimension at least $d$ (as complete positivity coincides with the positivity of the map $\Phi\otimes\idO_d$). In this way, the trace distance needs one extra dimension than the minimum in order to witness non-Markovianity. A similar result actually holds also for classical systems. In this case, one only needs to enlarge the state space by one extra dimension. Then, for any vector $\boldsymbol{v}$ on the original space, one can always construct a traceless state on this extended space as:
\begin{align}
	\delta\rho = \begin{cases}
		\delta\rho_i = v_i & {\rm if }\;i\in\curbra{1,\dots,d}\,;\\
		\delta\rho_{i}=-\sum_{j=1}^{d}\delta\rho_j & {\rm if }\;i\equiv d+1\,.
	\end{cases}
\end{align}
This state satisfies $\Tr{|\delta\dot{\rho}|} = \Tr{|\dot{\boldsymbol{v}}|}$, which proves the claim. Still, in this case it should be noticed that this construction cannot be carried out by adjoining an ancilla, as in that case the minimum dimension of the state space is $d_A=2$. Nonetheless, this example is useful as it shows that two dimensional ancillas are enough, and that in principle it would be sufficient to embed the dynamics $\Phi_t$ in a space only one dimension bigger than the original space in order to witness non-Markovianity.

\section{Detailed balance in the quantum regime}\label{app:sec:DB}

In this appendix we will first prove Thm.~\ref{cf:thm:eqDB} and then we will provide the structural characterisation of Fisher detailed balance Lindbladians presented in Eq.~\eqref{cf:eq:structAS}. 

Due to the amount of different notions of adjoints used in the following, we remind the reader about the notation used. There are three different scalar product used, namely the Hilbert-Schmidt one, $K_\pi^o$ and $K_{f,\pi}$, which induce the following adjoints:
\begin{align}
	\text{Hilbert}&\text{-Schmidt:}  \qquad \;\;\Tr{A X(B)}=\Tr{X^\dagger(A) B}\,;\label{eq:appHS}\\
	&K_\pi^o: \qquad\qquad \;\;\,\Tr{A O(B)\pi} = \Tr{\widetilde{O}^o(A) B\pi}\,;\label{eq:appAlickiProduct}\\
	&K_{f,\pi}: \qquad \qquad\Tr{A \J_f^{-1}[\mathcal{O} B]} = \Tr{(\widetilde{\mathcal{O}}_f A) \J_f^{-1}[ B]}\,,\label{eq:appASProduct}
\end{align}
where $O$ and $\mathcal{O}$ are a superoperator on the space of observables or on the state space, respectively, while $X$ is a generic bounded operator. As it is explained in the main text, one can formulate the adjoint with respect to $K_\pi^o$ or $K_{f,\pi}$ in terms of the Hilbert-Schmidt adjoint, thanks to the relation:
\begin{align}
	&\widetilde{O}^o = \RR_\pi^{-1}\circ O^\dagger\circ\RR_\pi\,;\\
	&\widetilde{\mathcal{O}}_f  =  \J_f\big|_{\pi}\circ \mathcal{O}^\dagger\circ \J_f^{-1}\big|_{\pi}\,,
\end{align}
as it can be verified directly from the definition. From this relations it is easy to see that the self-adjoint condition corresponds to the two equality $\RR_\pi\circ O= O^\dagger\circ\RR_\pi$ in the $K^o_\pi$ case, and $\mathcal{O}\circ\J_f\big|_{\pi} = \J_f\big|_{\pi}\circ \mathcal{O}^\dagger$ for the Fisher one. Thanks to this characterisation we can prove the following useful result:
\begin{lemma}\label{appM:lem:equivalence_when_commuting} 
	Suppose $\mathcal{O}$ and $O$ are adjoint of each other, $\mathcal{O}^\dagger \equiv O$. Then, if $[\mathcal{O},\LL_\pi\RR_\pi^{-1}]=0$, the two conditions of self-adjointness and skew-self-adjointness with respect to $K_{f,\pi}$ and $K_\pi^o$ coincide.
\end{lemma}
\begin{proof}
	First of all, it should be noticed that both the auto-modular operator $(\LL_\pi\RR_\pi^{-1})^\dagger = \LL_\pi^{-1}\RR_\pi = (\LL_\pi\RR_\pi^{-1})^{-1}$ and $(\RR_\pi)^\dagger = \LL_\pi$. Using these property we can show that the (skew-)self-adjointness with respect to $K_{f,\pi}$ is equivalent to the corresponding notion for  $K_\pi^o$. In fact, the following relations are equivalent:
	\begin{align}
		&\widetilde{\mathcal{O}}_f = \pm \mathcal{O} \iff
		(\mathcal{O} \J_f\big|_{\pi})^\dagger = \pm\,\mathcal{O}\J_f\big|_{\pi}\; \iff \;\\
		&\iff\;f((\LL_\pi\RR_\pi^{-1})^{-1}) \LL_\pi O = \pm\,\mathcal{O} \RR_\pi f(\LL_\pi\RR_\pi^{-1})   \; \iff\\
		&\iff\; \cancel{f(\LL_\pi\RR_\pi^{-1}) }\RR_\pi O = \pm\,\cancel{f(\LL_\pi\RR_\pi^{-1})} O^\dagger  \RR_\pi \iff\; \widetilde{O}^o = \pm O \,,
	\end{align}
	where in the last line we used the property $f(x) = x f(x^{-1})$, together with the commutation between $\mathcal{O}$ and $\LL_\pi\RR_\pi^{-1}$ to push $f(\LL_\pi\RR_\pi^{-1})$ to the left of both equations. Finally, the last step is simply the definition of $\mathcal{O}^\dagger \equiv O$.
\end{proof} 

This lemma is particularly useful because it allows to reduce the question about the equivalence of Def.~\ref{cf:def:alicki} and Def.~\ref{cf:def:AS} to the decision about the commutation of the Lindbladian with the auto-modular operator $\LL_\pi\RR_\pi^{-1}$.

\subsection{Proof of Theorem~\ref{cf:thm:eqDB}}

The aim of this section is to prove Thm.~\ref{cf:thm:eqDB}:

\begin{theorem*}
	The following conditions are equivalent:
	\begin{enumerate}
		\item  the generator of the dynamics in the Heisenberg picture $\lind^\dagger$ satisfies the adjointness relations in Def.~\ref{cf:def:alicki}\;\label{appM:cond:al}
		\item the Lindbladian $\lind$ satisfies the structural characterisation in Def.~\ref{cf:def:breuer}.\label{appM:cond:breuer}
		\setcounter{counterN}{\value{enumi}}
	\end{enumerate}
	These conditions imply:
	\begin{enumerate}
		\setcounter{enumi}{\value{counterN}}
		\item the generator of the dynamics in the Schroedinger picture $\lind$ satisfies the adjointness relations in Def.~\ref{cf:def:AS}.\label{appM:cond:AS}
	\end{enumerate}
	Moreover, if the Hamiltonian $H$ is non-degenerate the three conditions are equivalent.
\end{theorem*}

First, it should be noticed that the equivalence between condition~\ref{appM:cond:al} and~\ref{appM:cond:breuer} was already proven by Alicki in~\cite{alicki1976detailed}, so we postpone the proof to App.~\ref{appM:sec:structuralCh} where the characterisation of Lindbladians satisfying condition~\ref{appM:cond:AS} is given. In the particular case in which $H$ is non-degenerate, this will provide a proof of the structural definition of condition~\ref{appM:cond:breuer}.  

\begin{proof}
	First it should be noticed that if condition~\ref{appM:cond:breuer} is satisfied, the Lindbladian commutes with the auto-modular operator $\LL_\pi\RR_\pi^{-1}$. In fact, starting from the characterisation:
	\begin{align}
		\lind(\rho)=-i[H,\rho]+\sum_{\omega, i} \;\lambda_{i}^\omega \left(A_i^{\omega}\,\rho \,(A_i^{\omega})^\dagger -\frac{1}{2}\{(A_i^{\omega})^\dagger A_i^{\omega},\rho \} \right)\,,
	\end{align}
	it is a matter of straightforward calculations to verify that:
	\begin{align}
		\LL_\pi\RR_\pi^{-1}(\lind(\rho))&=-i\pi[H,\rho]\pi^{-1}+\sum_{\omega, i} \;\lambda_{i}^\omega \left((\pi\,A_i^{\omega}\pi^{-1})\,\pi\,\rho \,\pi^{-1}(\pi^{-1}A_i^{\omega}\,\pi)^\dagger -\frac{1}{2}\pi\{(A_i^{\omega})^\dagger A_i^{\omega},\rho \}\pi^{-1} \right)=\\
		&= -i[H,\pi\rho\pi^{-1}]+\sum_{\omega, i} \;\lambda_{i}^\omega \left(\cancel{e^{\omega}}\cancel{e^{-\omega}}\,A_i^{\omega}\,\pi\,\rho \,\pi^{-1}(A_i^{\omega})^\dagger -\frac{1}{2}\{(A_i^{\omega})^\dagger A_i^{\omega},\pi\,\rho\pi^{-1} \} \right)=\\
		&=\lind(\LL_\pi\RR_\pi^{-1}(\rho))
	\end{align}
	where we used the condition $[H,\pi]=0$, together with $\LL_\pi\RR_\pi^{-1}(A_i^\omega) = e^\omega \, A_i^{\omega}$ and $(A_i^{\omega})^\dagger = A_i^{-\omega}$. Since condition~\ref{appM:cond:breuer} is equivalent to condition~\ref{appM:cond:al}, and $[\mathcal{L},\LL_\pi\RR_\pi^{-1}]=0$, thanks to Lemma~\ref{appM:lem:equivalence_when_commuting} this means that $\lind$ has the same self-adjointness properties with respect to $K_\pi^o$ and $K_{f,\pi}$. This proves the forward implication.
	
	Let us prove the reverse, namely that condition~\ref{appM:cond:AS} is equivalent to condition~\ref{appM:cond:al} for non-degenerate Hamiltonians. Let us first focus on the unitary part. Then, using $\mathcal{U}^\dagger = -\mathcal{U}$ we can rewrite the skew-adjointness condition as:
	\begin{align}
		\mathcal{U} \circ\J_f\big|_{\pi} = -\J_f\big|_{\pi}\circ \mathcal{U}^\dagger \qquad \iff\qquad\mathcal{U} \circ\J_f\big|_{\pi} = \J_f\big|_{\pi}\circ \mathcal{U}\,.
	\end{align}
	Then, applying the two operators in the last equation to the identity, we can verify that:
	\begin{align}
		\mathcal{U} \circ\J_f\big|_{\pi}(\id) = \J_f\big|_{\pi}\circ \mathcal{U}(\id) &\implies \mathcal{U}(\pi) = -i\,\J_f\big|_{\pi}([H,\id]) \implies\\
		&\implies [H,\pi] = 0\,.\label{appM:eq:commU}
	\end{align}
	Notice that this result is generic, i.e., no assumptions on the spectrum of $H$ need to be made. This directly implies the commutation $[\mathcal{U},\LL_\pi\RR_\pi^{-1}]=0$, so again thanks to Lemma~\ref{appM:lem:equivalence_when_commuting} we have that  for the unitary part condition~\ref{appM:cond:AS} and~\ref{appM:cond:al} are always equivalent.
	
	Let us now focus on Eq.~\eqref{appM:eq:commU}. Since $H$ and $\pi$ commute, we can find a common set of eigenvectors, which we denote by $\{\ket{\alpha}\}$. Moreover, the basis $\{\ket{\alpha}\bra{\beta}\}$ gives a set of common eigenvectors to $\mathcal{U}$ and $\LL_\pi\RR_\pi^{-1}$, as it can be verified by direct calculation:
	\begin{align}
		&\mathcal{U}(\ket{\alpha}\bra{\beta})=-i(H_\alpha-H_\beta)\ket{\alpha}\bra{\beta}\,; \\
		& \LL_\pi\RR_\pi^{-1}(\ket{\alpha}\bra{\beta})=\frac{\pi_\alpha}{\pi_\beta}\ket{\alpha}\bra{\beta} \, .
	\end{align}
	Both superoperators have constant eigenvalues for all eigenvectors of the form $\ket{\alpha}\bra{\alpha}$. Under the assumption of continuity under small perturbations, we can also assume that each eigenvector such that $\alpha\neq\beta$ has a different eigenvalue (non-degenerate gap condition). These two observations together then imply that any superoperator commuting with $\mathcal{U}$ needs to commute with $\LL_\pi\RR_\pi^{-1}$ as well. In the main text we showed how normality of $\lind$ implies $[\mathcal{U},\lind_\mathcal{D}]=0$. Then, thanks
	to the considerations above, we also have that:
	\begin{align}
		[\lind_\mathcal{D},\LL_\pi\RR_\pi^{-1}]=0\ .\label{appM:eq:106}
	\end{align}
	Hence we can use Lemma~\ref{appM:lem:equivalence_when_commuting}, which implies that if $(\widetilde{\lind_\mathcal{D}})_f=\lind_\mathcal{D}$, we  also have that $(\widetilde{\lind_\mathcal{D}^\dagger})^o=\lind_\mathcal{D}^\dagger $. This concludes the proof.
\end{proof}

It should be noticed that the non-degeneracy of the spectrum is needed to prove the commutation relation in Eq.~\eqref{appM:eq:106}. The same equivalence can be proven if $\LL_\pi\RR_\pi^{-1}$ has some functional dependence on $\mathcal{U}$. Take for example the thermal scenario, i.e., $\pi\propto \exp[-\beta H]$. Then the auto-modular operator takes the form $\LL_\pi\RR_\pi^{-1}=\exp[-i\beta \mathcal{U}]$. Due to normality of the Lindbladian (which implies $[\mathcal{U},\lind_\mathcal{D}]=0$), we directly obtain Eq.~\eqref{appM:eq:106}, proving the equivalence without further assumptions on the spectrum of $\pi$ or $H$.

\subsection{Def.~\ref{cf:def:AS} is weaker in general}

Whereas the constraint coming from Def.~\ref{cf:def:alicki} imply the one in Def.~\ref{cf:def:AS}, the reverse does not hold in general. In fact, this is connected with the commutation between $\lind_\mathcal{D}$ and $\LL_\pi\RR_\pi^{-1}$. Whereas in the first definition of detailed balance these two operators always commute, this is not the case for the Fisher detailed balance dissipators. This leads to a less constrained evolution of the coherences, as it will be shown in the following.

First, as it was discussed in the proof in the previous section, if $\{\ket{\alpha}\}$ is an eigenbasis for $\pi$, then $\{\ket{\alpha}\bra{\beta}\}$ are eigenvectors for $\LL_\pi\RR_\pi^{-1}$, with eigenvalues:
\begin{align}
	\LL_\pi\RR_\pi^{-1}(\ket{\alpha}\bra{\beta})=\frac{\pi_\alpha}{\pi_\beta}\ket{\alpha}\bra{\beta} \, .
\end{align}
Since the steady state $\pi$ is always assumed to be full rank, proving that $\lind_\mathcal{D}$ commutes with $\LL_\pi\RR_\pi^{-1}$ is equivalent to requiring that the matrix elements
\begin{align}
	(\lind_\mathcal{D})_{\delta|\beta}^{\gamma|\alpha}\equiv\bra{\gamma}\lind_\mathcal{D}(\ketbra{\alpha}{\beta})\ket{\delta}
\end{align}
satisfy the following condition
\begin{align}
	[\lind_\mathcal{D},\Phi_\pi]=0 \quad\iff\quad 	(\lind_\mathcal{D})_{\delta|\beta}^{\gamma|\alpha}\left(\frac{\pi_\alpha}{\pi_\beta} -\frac{\pi_\gamma}{\pi_\delta}\right)=0\,.
\end{align}
Equivalently, this means that matrix elements of $\mathcal{D}$ can be nonzero only if:
\begin{align}
	\label{appM:eq:D_comm_coordinates}
	(\lind_\mathcal{D})_{\delta|\beta}^{\gamma|\alpha}\neq 0 \quad\implies\quad \frac{\pi_\alpha}{\pi_\beta} =\frac{\pi_\gamma}{\pi_\delta}\,.
\end{align}

In the following we show that a slightly more general condition follows from the requirement that $(\widetilde{\lind_\mathcal{D}})_f  = \lind_\mathcal{D}$ for all standard monotone functions $f$. Indeed, this condition can be written in coordinates as:
\begin{align}
	\lind_\mathcal{D}&\circ\J_f\big|_{\pi} = \J_f\big|_{\pi}\circ \lind_\mathcal{D}^\dagger \quad\iff\quad (\lind_\mathcal{D})^{\gamma|\alpha}_{\delta|\beta}\, f\norbra{\frac{\pi_\alpha}{\pi_\beta}}\pi_\beta  = (\lind_\mathcal{D})_{\alpha|\gamma}^{\beta|\delta}\,f\norbra{\frac{\pi_\gamma}{\pi_\delta}}\pi_\delta\,.
	\label{appM:eq:coordinateExpression}
\end{align}
At this point it is useful to introduce the notation $e^{-\omega_1} := \pi_\alpha/\pi_\beta$, and $e^{-\omega_2} := \pi_\gamma/\pi_\delta$.
Grouping the functional dependence on one side of the equation we obtain:
\begin{align}
	\frac{(\lind_\mathcal{D})^{\gamma|\alpha}_{\delta|\beta}\;\pi_\beta}{(\lind_\mathcal{D})_{\alpha|\gamma}^{\beta|\delta}\;\pi_\delta}  = \frac{f\norbra{e^{-\omega_2}}}{f\norbra{e^{-\omega_1}}}\,.\label{appM:eq:coordinateExpression2}
\end{align}
It should be noticed that the left hand side of the equation does not depend on the function $f$, so the coordinates of $\lind_\mathcal{D}$ are zero unless $\omega_1=\pm\omega_2$. Notice that the second condition follows from the symmetry of standard monotone functions $f(x) = x\,f(x^{-1})$.

Hence, the only non-zero elements of  $\lind_\mathcal{D}$ are satisfy either of the conditions:
\begin{align}
	\label{appM:eq:D_prop_or}
	(\lind_\mathcal{D})^{\gamma|\alpha}_{\delta|\beta}\neq 0 \implies
	\left(\frac{\pi_\alpha}{\pi_\beta}=\frac{\pi_\gamma}{\pi_\delta}\right) 
	\lor  
	\left(\frac{\pi_\alpha}{\pi_\beta}=\frac{\pi_\delta}{\pi_\gamma}\right)\, .
\end{align}
Comparing this result with Eq.~\eqref{appM:eq:D_comm_coordinates} directly shows that $\lind_\mathcal{D}$ does not commute in general with $\LL_\pi\RR_\pi^{-1}$, so Def.~\ref{cf:def:AS} is weaker than Def.~\ref{cf:def:alicki} (at the end of the section we present an explicit example showing this). For this reason, it is interesting to explore which constraints Eq.~\eqref{appM:eq:D_prop_or} imposes on the Lindbladian. First, it should be noticed that since $\lind_\mathcal{D}$ is adjoint preserving, its coordinates satisfy 
\begin{align}
	\label{appM:eq:D_prop_dagger}
	\lind_\mathcal{D}(A^\dagger)=\lind_\mathcal{D}(A)^\dagger 
	\quad \iff \quad
	(\lind_\mathcal{D})^{\gamma|\alpha}_{\delta|\beta}=(\bar{\lind}_\mathcal{D})_{\gamma|\alpha}^{\delta|\beta} \,.
\end{align}
Then, combining Eq.~\eqref{appM:eq:coordinateExpression2}, Eq.~\eqref{appM:eq:D_prop_or}, and Eq.~\eqref{appM:eq:D_prop_dagger}, we can see that:
\begin{itemize}
	\item populations and coherences do not mix, and the populations on the diagonal satisfy the classical detailed balance. In fact, from Eq.~\eqref{appM:eq:D_prop_or} we see that from $\alpha=\beta$ it follows that $\gamma=\delta$ (assuming $\pi$ to be non-degenerate), and the currents are related by the standard detailed balance condition:
	\begin{align}
		(\lind_\mathcal{D})^{\gamma|\alpha}_{\gamma|\alpha}\,\pi_\alpha=(\lind_\mathcal{D})^{\alpha|\gamma}_{\alpha|\gamma}\,\pi_\gamma\,.
	\end{align}
	\item The dynamics of the coherences can be split in two cases: the one for which  $\frac{\pi_\alpha}{\pi_\beta}=\frac{\pi_\gamma}{\pi_\delta}$, implying the following relation: 
	\begin{align}
		\label{appM:eq:old_case}
		(\lind_\mathcal{D})^{\gamma|\alpha}_{\delta|\beta}\,\pi_\beta =
		(\lind_\mathcal{D})^{\beta|\delta}_{\alpha|\gamma}\,\pi_\delta
		=(\bar{\lind}_\mathcal{D})_{\beta|\delta}^{\alpha|\gamma}\,\pi_\delta\, .
	\end{align}
	This property is satisfied also in the Alicki's definition of detailed balance.
	\item Moreover, one has additional transitions between coherences with characterised by the relation $\frac{\pi_\alpha}{\pi_\beta}=\frac{\pi_\delta}{\pi_\gamma}$.
	In this case the rate are given by:
	\begin{align}
		\label{appM:eq:new_case}
		(\lind_\mathcal{D})^{\gamma|\alpha}_{\delta|\beta}\,\pi_\beta =
		(\lind_\mathcal{D})^{\beta|\delta}_{\alpha|\gamma}\,\pi_\gamma
		=(\bar{\lind}_\mathcal{D})_{\beta|\delta}^{\alpha|\gamma}\,\pi_\gamma\, .
	\end{align}
	These rates are the only novelty compared with the one coming from Def.~\ref{cf:def:alicki}, and are the cause of the failure of $\lind_\DD$ from commuting with $\LL_\pi\RR_\pi$.
\end{itemize}

In order to justify the preference for Def.~\ref{cf:def:AS} as the quantum generalisation of detailed balance, we argue here that this last case is still physically sensible. Consider indeed two coherences terms $\ket{\alpha}\bra{\beta}$ and   $\ket{\gamma}\bra{\delta}$ such that $\frac{\pi_\alpha}{\pi_\beta}=\frac{\pi_\gamma}{\pi_\delta}$. Then, from Eq.~\eqref{appM:eq:old_case} it follows that the ratio between the currents induced between the two coherences is given by:
\begin{align}
	\frac{\big|(\lind_\mathcal{D})^{\gamma|\alpha}_{\delta|\beta}\big|}{\big|(\bar{\lind}_\mathcal{D})_{\beta|\delta}^{\alpha|\gamma}\big|}=
	\frac{\pi_\delta}{\pi_\beta}=\frac{\pi_\gamma}{\pi_\alpha}\, .\label{appM:eq:118}
\end{align}
The additional freedom given by  Eq.~\eqref{appM:eq:new_case} corresponds to  the possibility of the matrix element $(\lind_\mathcal{D})^{\delta|\alpha}_{\gamma|\beta}$ to be non-zero. It should be noticed, though, that the current between the two coherences is consistent with Eq.~\eqref{appM:eq:118}:
\begin{align}
	\frac{\big|(\lind_\mathcal{D})^{\delta|\alpha}_{\gamma|\beta}\big|}{\big|(\bar{\lind}_\mathcal{D})^{\alpha|\delta}_{\beta|\gamma}\big|}=
	\frac{\pi_\delta}{\pi_\beta}=\frac{\pi_\gamma}{\pi_\alpha}\, .\label{appM:eq:123c}
\end{align}
Thus, the difference between Def.~\ref{cf:def:alicki} and the Fisher one (i.e., Def.~\ref{cf:def:AS}), is that the first allows the coherences $\ket{\alpha}\bra{\beta}$ and   $\ket{\gamma}\bra{\delta}$ to communicate but prohibits interaction between $\ket{\alpha}\bra{\beta}$ and   $\ket{\delta}\bra{\gamma}$, while the latter allows the dynamics to connect  both off-diagonal elements, while keeping the ratio between the two currents detailed balanced.

Finally, before moving on to the characterisation of the Lindbladian operators satisfying Def.~\ref{cf:def:AS} we present here an example of $\lind$ which is detailed balance in the Fisher sense, but not according to Def.~\ref{cf:def:alicki}. Consider a two-levels system thermalizing to the Gibbs state
\begin{align}
	\pi_\beta=\frac{\ketbra{0}{0}+e^{-\beta}\ketbra{1}{1}}{1+e^{-\beta}}\, .
\end{align}
We consider the Hamiltonian of the system to be completely degenerate, i.e., $H\propto \id$, which implies $\mathcal{U}=0$. Then, it is easy to see that the Lindbladian  
\begin{align}
	\mathcal{L}(\rho)=A\rho A^\dagger -\frac{1}{2}\{\rho,A^\dagger A\}\,,
\end{align}
with the jump operator given by $ A=\ketbra{0}{1} + \sqrt{e^{-\beta}}\ketbra{1}{0}$ satisfies $\widetilde{\lind}_f=\lind$, but not $\widetilde{\lind}^o=\lind$.

\subsection{Structural characterisation of Def.~\ref{cf:def:AS}}\label{appM:sec:structuralCh}

This section is devoted to the derivation of the structural form of a detailed balanced Lindbladian according to the Def.~\ref{cf:def:AS}. Restricting the derivation to the case in which $\lind$ commutes with $\LL_\pi\RR^{-1}_\pi$ also proves the equivalence between 
Def.~\ref{cf:def:alicki} and Def.~\ref{cf:def:breuer}.

With the hindsight of the previous section it is useful to expand the Lindbladian operator in terms of the following eigenbasis:
\begin{align}
	F^\omega_\alpha := \curbra{\ketbra{\gamma}{\alpha}\bigg|\; \frac{\pi_\gamma}{\pi_\alpha} = e^{\omega}}\,.\label{appM:eq:a122}
\end{align}
It is also useful to introduce the function $\beta_\alpha(\omega) := \curbra{\beta|\, \pi_\beta = \pi_\alpha e^{\omega}}$, namely a function that returns the index $\beta$ such that $\frac{\pi_\beta}{\pi_\alpha} = e^\omega$. In order to keep the notation clear we also define $\gamma_\alpha(\omega)$ and $\delta_\alpha(\omega)$ exactly in the same way. The elements of the eigenbasis in Eq.~\eqref{appM:eq:a122} have the property that:
\begin{align}
	&(F^\omega_\alpha)^\dagger = F^{-\omega}_{\gamma_\alpha(\omega)}\,;\\
	&\pi F^\omega_\alpha = e^{\omega} \,F^\omega_\alpha \,\pi\,.
\end{align}
Generically, one can express the action of the dissipator as:
\begin{align}
	\lind_\mathcal{D}(\rho) :&= \sum_{\substack{\alpha, \beta,\\\gamma,\delta}}\; (\lind_\mathcal{D})^{\gamma|\alpha}_{\delta|\beta}\; \ketbra{\gamma}{\alpha}\, \rho \,(\ketbra{\delta}{\beta})^\dagger =\\
	&=\sum_{\substack{\alpha, \omega,\\\omega_1,\omega_2}}\; (\lind_\mathcal{D})^{\gamma_\alpha(\omega)|\alpha}_{\delta_\alpha(\omega+ \omega_2)|\beta_\alpha(\omega_1)}\; F^{\omega}_\alpha\, \rho \,(F^{\omega-\omega_1+\omega_2}_{\beta_\alpha(\omega_1)})^\dagger\,,
\end{align}
where we implicitly defined $ \pi_\gamma/\pi_\alpha=:e^{\omega}$, $ \pi_\beta/\pi_\alpha =: e^{\omega_1}$ and $\pi_\delta/\pi_\gamma =: e^{\omega_2}$. This expression is particularly useful because it allows for a straightforward  application of the constraints in Eq.~\eqref{appM:eq:D_prop_or}. In fact, we have that:
\begin{align}
	\frac{\pi_\alpha}{\pi_\beta}=\frac{\pi_\gamma}{\pi_\delta}\qquad&\iff\qquad \omega_1 = \omega_2\,;\\
	\frac{\pi_\alpha}{\pi_\beta}=\frac{\pi_\delta}{\pi_\gamma}\qquad&\iff\qquad \omega_1 = -\omega_2 \,.
\end{align}
Hence, the sum above can be restricted to the case $\omega_1 = \pm \omega_2$, giving:
\begin{align}
	\lind_\mathcal{D}(\rho) =&\sum_{\substack{\alpha,\omega\\\omega_1}}\; (\lind_\mathcal{D})^{\gamma_\alpha(\omega)|\alpha}_{\delta_\alpha(\omega+ \omega_1)|\beta_\alpha(\omega_1)}\; F^{\omega}_\alpha\, \rho \,(F^{\omega}_{\beta_\alpha(\omega_1)})^\dagger + \sum_{\substack{\alpha, \omega,\\\omega_1\neq 0}}\; (\lind_\mathcal{D})^{\gamma_\alpha(\omega)|\alpha}_{\delta_\alpha( \omega-\omega_1)|\beta_\alpha(\omega_1)}\; F^{\omega}_\alpha\, \rho \,(F^{\omega-2\omega_1}_{\beta_\alpha(\omega_1)})^\dagger\,.\label{eq:dissipatorSplit}
\end{align}
It should be noticed that the case $\omega_1 =0 $ is included in the first sum, so that we have to impose the constraint $\omega_1 \neq0 $ in the second line.
In this way $\lind_\DD$ naturally splits in two parts, $\lind_{\DD_1}$ (i.e., the operator in the first line) corresponding to the component of the dissipator commuting with $\LL_\pi\RR_\pi^{-1}$, and $\lind_{\DD_2}$, given by the sum in the second line. Interestingly, the condition $\widetilde\lind_\DD^o = \lind_\DD$ implies $\lind_\DD \equiv\lind_{\DD_1}$, so characterising the latter provides the structural form of detailed balance Lindbladian according to Def.~\ref{cf:def:alicki}. 

Whereas $\lind_{\DD_1}$ directly commutes with $\LL_\pi\RR_\pi^{-1}$, we can apply a transformation to $\lind_{\DD_2}$ to make it commuting. In particular, it should be noticed that $\lind_{\DD_2}$ transforms under the transposition superoperator $T$ as:
\begin{align}
	T\,\lind_{\DD_2}(\rho) &= \sum_{\substack{\alpha, \omega,\\\omega_1\neq 0}}\; (\lind_\mathcal{D})^{\gamma_\alpha(\omega)|\alpha}_{\delta_\alpha( \omega-\omega_1)|\beta_\alpha(\omega_1)}\; \norbra{F^{\omega}_\alpha\, \rho \,(F^{\omega-2\omega_1}_{\beta_\alpha(\omega_1)})^\dagger}^T =\\
	&= \sum_{\substack{\alpha, \omega,\\\omega_1\neq 0}}\; (\lind_\mathcal{D})^{\gamma_\alpha(\omega)|\alpha}_{\delta_\alpha( \omega-\omega_1)|\beta_\alpha(\omega_1)}\; \ketbra{\pi_\alpha e^{\omega-\omega_1}}{\pi_\alpha} \rho \ketbra{\pi_\alpha e^{\omega_1}}{\pi_\alpha e^{\omega}} = \\
	&=\sum_{\substack{\alpha, \omega,\\\omega_1\neq 0}}\; (\lind_\mathcal{D})^{\gamma_\alpha(\omega)|\alpha}_{\delta_\alpha( \omega-\omega_1)|\beta_\alpha(\omega_1)}\; F^{\omega-\omega_1}_\alpha\, \rho \,(F^{\omega-\omega_1}_{\beta_\alpha(\omega_1)})^\dagger=\\
	&=\sum_{\substack{\alpha, \omega,\\\omega_1\neq 0}}\; (\lind_\mathcal{D})^{\gamma_\alpha(\omega+\omega_1)|\alpha}_{\delta_\alpha( \omega)|\beta_\alpha(\omega_1)}\; F^{\omega}_\alpha\, \rho \,(F^{\omega}_{\beta_\alpha(\omega_1)})^\dagger\,,\label{appMeq:d2Transpose}
\end{align}
where in the second line we used the abuse of notation $\ket{\pi_\alpha}$ for $\ket{\alpha}$, and in the last line we made an implicit change of variables. From  Eq.~\eqref{appMeq:d2Transpose} we can see that $T\lind_{\DD_2}$ takes a form completely analogous to $\lind_{\DD_1}$. For this reason, it directly follows that:
\begin{align}
	[T\lind_{\DD_2}, \LL_\pi\RR_\pi^{-1}] = 0\,.
\end{align}
This condition allows to lift the characterisation for $\lind_{\DD_1}$ to $\lind_{\DD_2}$, as it will be shown in the following.

We begin by studying $\lind_{\DD_1}$. Notice that the coordinates of $\lind_\DD$ are related by:
\begin{align}
	(\lind_\mathcal{D})^{\gamma_\alpha(\omega)|\alpha}_{\delta_\alpha(\omega+ \omega_1)|\beta_\alpha(\omega_1)} =e^\omega\, (\lind_\mathcal{D})_{\alpha|\gamma_\alpha(\omega)}^{\beta_\alpha(\omega_1)|\delta_\alpha(\omega+ \omega_1)}\,, \label{appM:eq:appRateRelations}
\end{align}
as it can be verified from Eq.~\eqref{appM:eq:coordinateExpression2}. Then, we can diagonalise $\lind_{\DD_1}$ in a way completely analogous to the procedure carried out in Sec.~\ref{cf:sec:markovRates}. To this end, it is useful to introduce a new basis of operators, given by $\curbra{X^\omega_m} = \curbra{\Delta_i}_{1\leq i\leq d}\cup \curbra{F^\omega_\alpha}_{\omega\neq0}$, where $\curbra{\Delta_i}_{1\leq i\leq d}$ is an orthonormal basis for the diagonal matrices, and $\Delta_1 = \id/\sqrt{d}$. Then, we can rewrite $\lind_{\DD_1}$ in this basis as:
\begin{align}
	\lind_{\DD_1}(\rho) &= \sum_{\substack{\alpha,\beta}}\; (\lind_\mathcal{D})^{\gamma_\alpha(0)|\alpha}_{\delta_\beta( 0)|\beta}\; F^{0}_\alpha\, \rho \,(F^{0}_{\beta})^\dagger+\sum_{\substack{\alpha,\beta\\\omega\neq 0}}\; (\lind_\mathcal{D})^{\gamma_\alpha(\omega)|\alpha}_{\delta_\beta(\omega)|\beta}\; F^{\omega}_\alpha\, \rho \,(F^{\omega}_{\beta})^\dagger =\\
	&=\sum_{\substack{i,j}}\; D_{i,j}^0\; \Delta_i\, \rho \,(\Delta_j)^\dagger+ \sum_{\substack{\alpha, \beta,\\\omega\neq 0}} \;D_{\alpha,\beta}^\omega\; F^{\omega}_\alpha\, \rho \,(F^{\omega}_{\beta})^\dagger\,,
\end{align} 
where we introduced the coefficients $D_{\alpha,\beta}^\omega:=(\lind_\mathcal{D})^{\gamma_\alpha(\omega)|\alpha}_{\delta_\beta(\omega)|\beta}$ and
\begin{align}
	D^0_{i,j} = \sum_{\alpha,\beta}\;(\lind_\mathcal{D})^{\alpha|\alpha}_{\beta|\beta}\, \bar{U}_{\alpha,i} \,U_{j,\beta}\,,
\end{align}
where $U$ is the unitary defined by $\Delta_i := U_{i,\alpha} F_\alpha$. In order to make the dissipator explicitly trace preserving, we highlight the terms containing the identity operator. In analogy to Sec.~\ref{cf:sec:markovRates} this leads to the form:
\begin{align}
	\lind_{\mathcal{D}_1}(\rho) =\curbra{K,\rho} +\sum_{\substack{i,j \neq (1,1)\\ \omega}} D^\omega_{i,j}\; X^\omega_i\, \rho \,(X_j^\omega)^\dagger\,,
\end{align}
and $K := \frac{D^0_{1,1}}{2 d}\id + \frac{1}{\sqrt{d}}\sum_i D^0_{i,1}\Delta_i$. The absence of the Hamiltonian contribution follows from the fact that we are looking at the dissipator alone. Equivalently, it is not hard to show that all the $D^0_{i,j}$ are indeed real. 

It should be noticed that $\lind_{\mathcal{D}_2}$ only gives contributions out of the diagonal, so one can impose trace preservation on $\lind_{\mathcal{D}_1}$ alone, i.e., $\lind_{\mathcal{D}_1}^\dagger(\id) = 0$. This directly implies that $K = -\frac{1}{2}\norbra{\sum_{\substack{i,j \neq (1,1)}} D^\omega_{i,j}(X_j^\omega)^\dagger X_i^\omega}$,  so the dissipator can be rewritten in Lindblad form: 
\begin{align}
	\lind_{\mathcal{D}_1}(\rho) = \sum_{\substack{i,j \neq (1,1)\\ \omega}} D^\omega_{i,j}\; \norbra{X_i^\omega\, \rho \,(X_j^\omega)^\dagger -\frac{1}{2}\curbra{(X_j^\omega)^\dagger X_i^\omega,\rho}}\,.\label{appM:eq:141}
\end{align}
The property of the dissipator of being adjoint preserving implies that the matrix $D^\omega_{i,j}$ is Hermitian. Then, there exists a unitary matrix $V$, such that $D^\omega_{i,j} = V^\omega_{i,m}(\lambda^\omega_m \delta^{m}_n)(V^\omega)_{n,j}^\dagger $, where we sum over repeated indexes. Hence, define the jump operators $A_m^\omega := X^\omega_i V^\omega_{i,m}$. Then, Eq.~\eqref{appM:eq:141} becomes:
\begin{align}\label{appM:eq:142}
	\lind_{\mathcal{D}_1}(\rho)  &= \sum_{\substack{i,j \neq (1,1)\\\omega}}\; \lambda^\omega_m \; V^\omega_{i,m}(V^\omega)_{m,j}^\dagger \norbra{X^\omega_i\, \rho \,(X^\omega_j)^\dagger -\frac{1}{2}\curbra{(X^\omega_j)^\dagger X^\omega_i,\rho}} = \\
	&=\sum_{m,\omega} \;\lambda^\omega_m \;\norbra{A^\omega_m\, \rho \,(A^\omega_m)^\dagger -\frac{1}{2}\curbra{(A^\omega_m)^\dagger A^\omega_m,\rho}}\,.
\end{align}
We can now characterise the properties of the jump operators and of the rates in the previous equation. First, it should be noticed that, since $X_i^\omega$ are eigenoperators of the  auto-modular operator $\LL_\pi\RR_\pi^{-1}$, the same holds for $A_m^\omega$, as the unitary does not mix $X_i^\omega$s  with different $\omega$s. Moreover, Eq.~\eqref{appM:eq:appRateRelations} implies that $D^\omega_{\alpha,\beta} = e^{\omega}\,D^{-\omega}_{\delta_\beta(\omega), \gamma_\alpha(\omega)}$, where we used the same indices as in the equation. This relation shows that $D^{-\omega}_{\delta_\beta(\omega), \gamma_\alpha(\omega)}$ can be diagonalised as $e^{-\omega}\lambda^{\omega}_m\delta_n^m =(V^\omega)_{m,\alpha}^\dagger D^{-\omega}_{\delta_\beta(\omega), \gamma_\alpha(\omega)}(V^\omega)_{\beta,n}$. We can deduce the following two facts: first, the spectrum of $D^\omega_{\alpha,\beta}$ satisfies $\lambda_{i}^\omega=e^{\omega}\,\lambda_{i}^{-\omega}$; second, since $(X^\omega_{\alpha})^\dagger = X^{-\omega}_{\gamma_\alpha(\omega)}$, it also holds that $(A^\omega_i)^\dagger = X^{-\omega}_{\gamma_\alpha(\omega)} (V^\omega_{\alpha,i})^\dagger = X^{-\omega}_{\gamma_\alpha(\omega)} V^{-\omega}_{\gamma_\alpha(\omega),i} = A^{-\omega}_i$. Hence, we see that $\lind_{\mathcal{D}_1}$ satisfies the same conditions of Def.~\ref{cf:def:breuer}, namely:
\begin{enumerate}%[label=(\roman*)]
	\item $(A_i^{\omega})^\dagger = A_i^{-\omega}$;
	\item $\pi \,A_i^{\omega}\, \pi^{-1}=e^{\omega}\, A_i^{\omega}$ ;
	\item $\lambda_{i}^\omega=e^{\omega}\,\lambda_{i}^{-\omega}$.
\end{enumerate}
Since $\lind_{\DD_1}$ is the only component of the dissipator if one uses Def.~\ref{cf:def:alicki}, this proves the equivalence between this notion of detailed balance and the structural characterisation in Def.~\ref{cf:def:breuer}.

We can now pass to characterise $\lind_{\mathcal{D}_2}$. Thanks to Eq.~\eqref{appMeq:d2Transpose} we can rewrite it as:
\begin{align}
	\lind_{\mathcal{D}_2}(\rho)&=\sum_{\substack{\alpha, \omega,\\\omega_1\neq 0}}\; (\lind_\mathcal{D})^{\gamma_\alpha(\omega+\omega_1)|\alpha}_{\delta_\alpha( \omega)|\beta_\alpha(\omega_1)}\;(F^{\omega}_\alpha\, \rho \,(F^{\omega}_{\beta_\alpha(\omega_1)})^\dagger)^T=\sum_{\substack{\alpha\neq\beta,\\\omega}}\; (\lind_\mathcal{D})^{\gamma_\beta(\omega)|\alpha}_{\delta_\alpha( \omega)|\beta}\;F^{\omega}_{\beta}\, \rho^T \,(F^{\omega}_\alpha)^\dagger =\\
	&=\sum_{\substack{\alpha\neq\beta,\\\omega}}\; (\lind_\mathcal{D})^{\delta_\beta(\omega)|\alpha}_{\gamma_\alpha( \omega)|\beta}\;F^{\omega}_{\beta}\, \rho^T \,(F^{\omega}_\alpha)^\dagger  \,,\label{appM:eq:144}
\end{align}
where we eliminated the dependence on $\omega_1$ by enforcing the constraint $\alpha\neq\beta$. Finally, in the last line we changed exchanged the dummy indexes $\gamma$ and $\delta$ to highlight the analogy with the other part of the Lindbladian. Indeed, define the matrix $\widetilde{D_{\alpha,\beta}^\omega}:= (\lind_\mathcal{D})^{\delta_\beta(\omega)|\alpha}_{\gamma_\alpha( \omega)|\beta}$ for any $\alpha\neq\beta$ and zero on the diagonal. It is interesting to compare it to the off-diagonal elements of $D_{\alpha,\beta}^\omega = (\lind_\mathcal{D})^{\gamma_\alpha(\omega)|\alpha}_{\delta_\beta( \omega)|\beta}$: as it can be seen, the two are related by an exchange $\gamma_\alpha(\omega)\leftrightarrow\delta_\beta(\omega)$. Moreover, thanks to Eq.~\eqref{appM:eq:123c} it also holds that:
\begin{align}
	\widetilde{D_{\alpha,\beta}^\omega}  = e^\omega\,\widetilde{D}_{\delta_\beta(\omega),\gamma_\alpha(\omega)}^{-\omega}\,,
\end{align}
which shows the analogy with $D_{\alpha,\beta}^\omega$  even further.  Using Eq.~\eqref{appM:eq:D_prop_dagger} it also follows that $\widetilde{D_{\alpha,\beta}^\omega}$ is hermitian, so there exist a unitary matrix $W$ such that  $\widetilde{D_{\alpha,\beta}^\omega} = W^\omega_{\alpha,m}(\mu^\omega_m \delta^{m}_n)(W^\omega)_{n,\beta}^\dagger $. We also define the jump operators $B_m^\omega := (W^\omega_{m,\alpha})^\dagger F^\omega_\alpha $. Then, one can rewrite $\lind_{\mathcal{D}_2}$ as:
\begin{align}
	\lind_{\mathcal{D}_2}(\rho)&= \sum_{\substack{\alpha\neq\beta,\\\omega}}\; W^\omega_{\alpha,m}(\mu^\omega_m \delta^{m}_n)(W^\omega)_{n,\beta}^\dagger \;F^{\omega}_{\beta}\, \rho^T \,(F^{\omega}_\alpha)^\dagger  =\\
	&= \sum_{m}\;\mu^\omega_m\,B_m^\omega \,\rho^T (B_m^\omega )^\dagger\,.
\end{align}
In analogy with the previous case it also holds that $\mu^\omega_i = e^\omega\mu^{-\omega}_i$ and $(B_m^\omega)^\dagger = B_m^{-\omega}$, together with the fact that $B_m^\omega$ is an eigenoperator of $\LL_\pi \RR_\pi^{-1}$. Still, there is one crucial difference with $\lind_{\mathcal{D}_1}$: since all the diagonal elements of $\widetilde{D_{\alpha,\beta}^\omega}$ are zero, this matrix is traceless, meaning that the sum of the eigenvalues is zero also zero. Hence, whereas $\lambda_i^\omega\geq0$ for all $i$ and $\omega$, we have the extra constraint $\sum_i \mu_i^\omega = 0 $, implying the negativity of some of the $\mu_i^\omega$. Putting everything together, we finally obtain the characterisation in Eq.~\eqref{cf:eq:structAS}.
